Learning a Complete Image Indexing Pipeline

To work at scale, a complete image indexing system comprises two components: An inverted file index to restrict the actual search to only a subset that should contain most of the items relevant to the query; An approximate distance computation mechanism to rapidly scan these lists. While supervised deep learning has recently enabled improvements to the latter, the former continues to be based on unsupervised clustering in the literature. In this work, we propose a first system that learns both components within a unifying neural framework of structured binary encoding.

==> figures/K3D3.tex <==

\begin{tikzpicture}
  \def\colA{2}
  \def\colB{2}
  \def\dx{0.4}
  \begin{axis}[
    scale only axis,
    width=0.7\columnwidth, height=0.5\columnwidth, 
    grid=none,
    ztick={1},xtick={1},ytick={1},
    axis lines=center,
    enlargelimits=true,        
    view={60}{30},
    %legend pos=south,
    legend style={at={(0.4,-.02)}, legend columns=-1, anchor=north, draw=none,
      /tikz/every even column/.append style={column sep=1em}}
    ]
    % \addplot3[surf, samples=2,shader=interp]{x+y};
    \addplot3[only marks,mark=*,red] coordinates {(1,0,0)(0,1,0)(0,0,1)};    
    \addplot3[patch, patch type=triangle, point meta=explicit, shader=interp,fill opacity=0.75,area legend,fill=blue,draw=black] coordinates
    {(1,0,0)[\colA] (1-\dx,\dx,0)[1] (1-\dx,0,\dx)[1]
      (0,1,0)[\colB] (\dx,1-\dx,0)[1] (0,1-\dx,\dx)[1]
      (0,0,1)[\colB] (\dx,0,1-\dx)[1] (0,\dx,1-\dx)[1] };
    % \addplot3[patch, patch type=polygon, shader=flat mean, faceted color=none, draw=none, vertex count=6,
    % point meta=explicit, fill opacity=0.75,area legend,fill=blue] coordinates
    % { (1-\dx,\dx,0)[1] (1-\dx,0,\dx)[1]
    %   (\dx,0,1-\dx)[1] (0,\dx,1-\dx)[1]
    %   (0,1-\dx,\dx)[1] (\dx,1-\dx,0)[1] 
    % };
    \addplot3[patch, patch type=triangle, shader=interp, 
    point meta=explicit, fill opacity=0.75,area legend,fill=red] coordinates
    { (1-\dx,\dx,0)[1] (1-\dx,0,\dx)[1] (\dx,0,1-\dx)[1]
      (1-\dx,\dx,0)[1] (\dx,0,1-\dx)[1] (0,\dx,1-\dx)[1]
      (1-\dx,\dx,0)[1] (0,\dx,1-\dx)[1] (0,1-\dx,\dx)[1]
      (1-\dx,\dx,0)[1] (0,1-\dx,\dx)[1] (\dx,1-\dx,0)[1] 
    };

    \legend{$\ms K_3$,$\Delta_3$,$p(\bmt b_m)$}

    % Labels
    %\node[below right, at (axis cs:0.45,0.45,0) {$\Delta_3$};


  \end{axis}
  
\end{tikzpicture}


%%% Local Variables:
%%% TeX-master: "../master.tex"
%%% End:

==> figures/_region_.tex <==
\message{ !name(subic.tex)}
\message{ !name(subic.tex) !offset(-2) }

\usetikzlibrary{positioning,arrows,fit,calc,shadows}
%% Diagonal fill
\tikzset{
  diagonal fill/.style 2 args={fill=#2, path picture={
      \fill[#1, sharp corners] (path picture bounding box.south west) -|
      (path picture bounding box.north east) -- cycle;}},
  reversed diagonal fill/.style 2 args={fill=#2, path picture={
      \fill[#1, sharp corners] (path picture bounding box.north west) |-
      (path picture bounding box.south east) -- cycle;}}}
%% Node styles
\tikzset{%
  block/.style={draw, fill=blue!20!white, rounded corners, rectangle,
    minimum height=2em, minimum width=2em, font=\footnotesize\scshape, align=center, drop shadow},
  W/.style={draw, rectangle, minimum height=1.5em, minimum width=1.5em, drop shadow, fill=white},
  bbox/.style={draw, rounded corners, dashed, rectangle},
  activ/.style={font=\tiny\itshape,at start,inner sep=2pt},
  fit label/.style={inner sep=.3em,font=\small\itshape},
  input/.style={inner sep=0pt},
  output/.style={inner sep=0pt},
  sum/.style = {draw, fill=white, circle, minimum size=.8em, node distance=5em, inner sep=0pt},
  pinstyle/.style = {pin edge={to-,thin,black}}
}

\begin{tikzpicture}[auto, node distance=4em and 4em, on grid, >=latex', font=\small]
  
  % Encoder
  \node[W, right=6em of softmax.east] (W2) {$\bm W_2$};
  \node[block, right=of W2.east](block softmax){Block\\SoftMax};
  \node[block, above=2em of block softmax.north](block one hot){Block\\One-Hot};
  \node[draw,inner sep=2mm,bbox, fit=(W2) (block softmax)](encoder) {};
  \node[above right, fit label] at (encoder.north west) {Encoder};

  % Encoder arrows
  \draw [->] (W2)  -- node[activ,above right]{ReLU} node[below]{$\bm z \in \R^{KM}_+$} (block softmax);
  %\draw [->] (W2) -- node[at start,activ,above right]{ReLU} (block softmax);
  \draw [->] ($(block softmax.west)-(1em,0)$) |- (block one hot);
  \draw [->] (block softmax.east) --  node[above right]{$\bmt{b} \in \Delta_{K}^M$}   +(2em,0) ;
  \draw [->] (block one hot.east) -- node[above right]{$\bm b \in \ms K_{K}^M$} +(2em,0);
  
\end{tikzpicture}

\message{ !name(subic.tex) !offset(-45) }

